Team-oriented Consistency Checking of Heterogeneous Engineering Artifacts

Consistency checking of interdependent heterogeneous engineering artifacts, such as requirements, specifications, and code, is a challenging task in large-scale engineering projects. The lack of team-oriented solutions allowing a multitude of project stakeholders to collaborate in a consistent manner is thus becoming a critical problem. In this context, this work proposes an approach for team-oriented consistency checking of collaboratively developed heterogeneous engineering artifacts.

==> sections/acknowledgement.tex <==
\section{Acknowledgement}
The research reported in this paper has been partly funded by the Austrian Science Fund (FWF) (grant \# P31989-N31 as well as grant \# I 4744-N), and the LIT Secure and Correct System Lab sponsored by the province of Upper Austria.
